Predicting passenger loading level on a train car: A Bayesian approach

Crowding in train cars is increasingly a major concern for transit agencies. From the perspective of the passengers and the transit agencies, overcrowding of the train cars has several negative consequences such as: (i) extended duration of passengers boarding and alighting which leads to longer dwell times, (ii) subsequent disruption of the headway and the schedule, and (iii) passenger dissatisfaction (e.g. increased stress and lack of privacy). Moreover, overcrowding during peak service hours also indicates inadequate infrastructure to meet the passenger demands. Realizing the importance of the crowding issue, transit agencies have developed measures to assess the crowding levels. The Transit Capacity and Quality of Service Manual provides guidelines on thresholds for crowding in transit systems in the United States.

==> accel_apc.tex <==
\chapter{Accelerometer based APC}
\label{ch:apc}
An automatic passenger counter (APC) is the main source of data for the CICD system. ARCON proposed to develop an accelerometer based APC to measure the passenger loading on train cars. The accelerometer based method would be an economical solution to automatic passenger counting compared to existing solutions. An accelerometer sensor can measure static acceleration like gravity or dynamic acceleration due to the motion or vibration. When properly attached to an object, an accelerometer can be used to measure the dynamic acceleration of the object. The goal of the proposed method is to infer the passenger loading level from the accelerometer measurements on-board a train car.

In classical mechanics, the acceleration of a body subjected to an external input force depends on the body mass. Changing the body mass changes the acceleration given that the same input force is applied. The change in acceleration can be measured using an accelerometer attached to the object. In the same spirit, the accelerometer-based APC is based on the idea that a train carbody vibration should change with changes in the carbody mass due to alighting and boarding passengers. These changes in carbody vibration can be measured using an accelerometer fixed onto the carbody.

The train carbody vibrations impact the ride quality and riders comfort. The allowed levels of vibrations are regulated by ISO 2631-1 standard. The train cars must be designed such that vibrations are minimized in the frequency bands that the passengers are most sensitive to. It was shown that the vertical vibrations have the most impact on riders comfort. A number of theoretical and experimental studies have been performed to measure the impact of vertical train car vibrations on the riders comfort. Among other results the authors in \cite{carlbom2000carbody, nagai2006coupled, tomioka2015experimental} report that the carbody vibration spectrum changes when the number of passengers change, and the effect is most noticeable in the frequency range of the carbody's first flexible vibration mode. Although the results of these studies focus on the ride quality, they confirm our intuition that it is possible to detect changes in the train carbody mass by measuring vertical vibrations.
 
One of the major goals of the Phase I effort is to demonstrate a PoC of using train car accelerometer data to implement an APC. This PoC also marks the first milestone of the Phase I effort. ARCON pursued a two-pronged approach to demonstrate the PoC for the accelerometer based APC:
\begin{description}
\item [Model analysis] This approach used simplified theoretical models for train carbody to analyze the relation between carbody mass and vertical vibration.  
\item [Data driven analysis] This approach focused on gathering accelerometer data from an operational train car and conducting analysis to establish the relation between passenger loading and the vibration measurements.
\end{description}
As a part of the two-pronged approach, ARCON successfully completed a series of theoretical and experimental analyses to establish a correlation between the carbody vertical vibration and the passenger loading. This correlation between the measurement and passenger loading demonstrates the proof-of-concept for using accelerometer data to estimate passenger loading on a train car. The sections below describe two approaches in detail.

\section{Model analysis approach}
A common approach when analyzing a complex system such as a train car is to start with a simplified theoretical model to build an initial insight. Train cars are usually modeled using simple mass-spring-damper systems with varying degrees-of-freedom (DOF). This simplified model allows us to analytically solve for the quantity of interest. For our purpose we are interested in deriving the relation between the train car vertical vibration and its mass. 

\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\textwidth]{carbody.png}
\caption{Train car consists of a carbody mounted on a pair of bogies.}
\label{fig:carbody}
\end{figure}

Figure~\ref{fig:carbody} shows a typical train car which consists of the carbody mounted on a pair of bogies \cite{carlbom2000carbody,garg2012dynamics}. The passengers board the carbody which is connected to the bogies via a secondary suspension system. Each bogie has a pair of wheels on either side resting on a pair of track rails (not shown in figure). The wheels are connected to the bogie via a primary suspension system. The wheels are assumed to follow the track geometry as the train car moves along the track. Any variation on the track geometry will vertically displace the wheels. This vertical displacement of the wheels are transmitted via the suspension system to the carbody. The vertical vibration of the carbody is a combined effect of the input from the track geometry variation transformed via the suspension systems and the mechanical response of the carbody. The track geometry variations are the primary dynamic inputs to the train car. For a train car moving with a constant velocity, the wheel displacement due to the track geometry variation can be viewed as a time-series input. The input from track geometry variation is commonly modeled as a periodically modulated stochastic process \cite[Section~3.8]{garg2012dynamics}.

The vertical vibration observed in the carbody is a combination of rigid body motion (bounce and pitch) and flexible bending motion. The rigid body motion is what is usually perceived by the train passengers as vibration. It is a slow shaking of the car up and down due to unevenness of tracks. The flexible body vibrations occur since the train car is not an ideal rigid body and it can experience a certain amount of bending and torsion. The vibration motion is spatially distributed along the carbody. The spatial distribution of the vibration can be resolved into different spatial mode shapes. Each mode shape has a different temporal frequency. The rigid modes and flexible modes exists in distinct frequency bands \cite{carlbom2000carbody,tomioka2015experimental}. This spectral separation of vertical vibration modes forms the basis for the spectral analysis of vertical vibration.

Two models were considered for the model based analysis. The first model was a simple 2-degrees-of-freedom (2-DOF) mass-spring-damper system. This model captures only the rigid mode motion, but provides a simple analytical solution for vertical vibration. The second model was a multi-DOF system which captures both rigid modes and flexible modes. The multi-DOF system is a more realistic model of a train car.

\subsection{2-DOF mass-spring-damper model}
Figure~\ref{fig:twodof_model} shows a 2-DOF mass-spring-damper system used as a model for the train car. The two mass units correspond to the carbody mass, $m_c$, and the bogie mass, $m_b$. The secondary suspension is modeled by a spring-damper system with spring constant, $k_c$, and damper coefficient, $c_c$. The bogie is assumed to have a single point contact with the track via the primary suspension. The primary suspension is modeled by the spring-damper system with spring constant, $k_b$, and damper coefficient, $c_b$. The entire model is assumed to be moving at a constant velocity, $v$. As the model moves forward, the primary suspension point contact is displaced vertically following the track geometry. The displacement of the point contact is denoted by $z_o$. This displacement due to the track irregularities is the only input applied to the model. The resulting displacement of the carbody mass and the bogie mass are denoted by $z_c$ and $z_b$ respectively.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.25\textwidth]{twodof_model.eps}
\caption{2-DOF spring-mass-damper model for train carbody excited by track irregularities.}
\label{fig:twodof_model}
\end{figure}

The 2-DOF model has two observable displacements and a single input in the form of the base displacement. Hence, the equations of motions are,
 \begin{align}
 \label{eq:2dof-eqmo}
 \masscar \ddot{z_c} + \ccar(\dot{z_c} - \dot{z_b}) + \kcar(z_c - z_b) =& 0 \nonumber \\ 
 \massbogie \ddot{z_b} + \ccar(\dot{z_b} - \dot{z_c}) + \kcar(z_b - z_c) + \cbogie\dot{z_b} + \kbogie z_b =& \cbogie\dot{z_o} + \kbogie z_o
 \end{align}
Our interest is in understanding how the carbody vertical displacement responds to the base excitation from the track. Using Eq.~\ref{eq:2dof-eqmo}, the transfer function between the carbody displacement, $z_c$, and the base displacement, $z_o$, is
 \begin{align}
 \label{eq:2dof_tf}
 \tf = \frac{\ccar\cbogie s^2 + (\ccar\kbogie + \cbogie\kcar)s + \kcar\kbogie}{\massbogie\masscar s^4 + (\ccar\massbogie + (\ccar-\cbogie)\masscar)s^3 + (\ccar\cbogie + \kcar\massbogie + (\kbogie - \kcar)\masscar)s^2 + (\ccar\kbogie + \cbogie\kcar)s + \kcar\kbogie}
 \end{align}
Eq.~\ref{eq:2dof_tf} relates the carbody displacement to the base excitation input and clearly shows that the carbody displacement response depends on the carbody mass. Figure~\ref{fig:twodof_tf} shows the transfer functions computed using the parameters in Table~\ref{tbl:2dof_parameters}. Each color corresponds to a different passenger loading level indicated in the legend. Each passenger is assumed to weigh 70kgs. Increasing the passenger count effectively increases the carbody mass and the transfer function also changes. Considering the transfer function at 1~Hz, it is observed that the transfer function magnitude decreases with increase in the passenger loading.

\begin{table}[!ht]
\centering
\caption{2-DOF model simulation parameters.}
\label{tbl:2dof_parameters}	
	\begin{tabular}{|r|l|}
    	\hline
         carbody mass($m_b$) & 38000kg \\
         %\hline         
         bogie mass ($m_t$) & 3000kg\\
         %\hline        
         primary suspension stiffness ($k_c$) & 0.78 $\times 10^6$~N/m\\
         %\hline
         secondary suspension stiffness ($k_b$) & 0.55 $\times 10^6$~N/m\\
         %\hline
         primary suspension damping ($c_c$) & 30 $\times 10^6$~Ns/m\\
         %\hline
         secondary suspension damping ($c_b$) & 60 $\times 10^3$~Ns/m\\
         mass per person & 70kg \\
         \hline
    \end{tabular}	
\end{table}

\begin{figure}[!ht]
\centering    
\includegraphics[width=0.7\textwidth]{twodof_tf.png}        
\caption{Carbody vertical displacement acceleration output to track input transfer function.}
\label{fig:twodof_tf}
\end{figure}      

\begin{figure}[!ht]
\centering
\includegraphics[width=0.7\textwidth]{fre_res_vs_mas_2.png}
\caption{Transfer function at a fixed frequency vs passenger loading}
\label{fig:twodof_fxfreqtf}   
\end{figure}

Figure~\ref{fig:twodof_fxfreqtf} shows how the transfer function magnitude at a particular frequency changes with increase in passenger loading. The x-axis corresponds to the passenger count and the y-axis corresponds to the transfer function magnitude ($|H(f_0)|$) evaluated at a fixed frequency $f_0$. Each curve corresponds to a different value of $f_0$ indicated in the legend. In all five frequency values considered in Figure~\ref{fig:twodof_fxfreqtf}, the transfer function magnitude decreases with increase in the passenger count. Clearly the change in carbody mass impacts the vertical vibration response of the carbody. This change in the carbody vibration due to change in passenger loading is the basis of the proposed accelerometer based APC. 

\subsection{Multi-DOF model}
\label{sec:mdof}
Multi-DOF models are used for higher fidelity representation of the carbody response \cite{garg2012dynamics}. Multi-DOF models can capture vibration due to both rigid body motion and flexible motion. For the purpose of Phase I task, we considered the multi-DOF model shown in Figure~\ref{fig:mdof_model}, in which only vertical vibrations are considered. In this model, the carbody is assumed to be a simple uniform Euler-Bernoulli beam supported by the secondary suspensions on the bogies. It is assumed that when the train car moves on the track, the wheels follow the track irregularities \cite{zhou2009influences}.
\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{carbody-model.png}
\caption{Multi-DOF model of train carbody mounted on two bogie units \cite{zhou2009influences}.}
\label{fig:mdof_model}
\end{figure}

\begin{table}[!ht]
\centering
\caption{Mutli-DOF model simulation parameters.}
\label{tb:sim-params}	
	\begin{tabular}{|r|l|}
    	\hline
         carbody mass($m_b$) & 28000\,kg \\
         %\hline
         carbody pitch inertia & 1.3 $\times 10^6$\,kg m\textsuperscript{2} \\
         %\hline
         carbody bending stiffness & 4.987 $\times 10^9$\,kN/m\textsuperscript{th}\\
         %\hline
         carbody internal damping coefficient& 1.936 $\times 10^6$\,kN s/m\textsuperscript{th}\\
         %\hline
         carbody length ($L$) & 24.5\,m\\
         %\hline
         bogie mass ($m_t$) & 2500\,kg\\
         %\hline
         bogie pitch inertia & 1500\,kg$\cdot$m\textsuperscript{th} \\
         %\hline
         half distance between bogies ($l_b$) & 8.75\,m\\
         %\hline
         half wheelbase & 1.25\,m\\
         %\hline
         primary suspension stiffness ($k_p$) & 2.4 $\times 10^6$\,N/m\\
         %\hline
         secondary suspension stiffness ($k_s$) & 0.5 $\times 10^6$\,N/m\\
         %\hline
         primary suspension damping ($c_p$) & 30 $\times 10^6$\,Ns/m\\
         %\hline
         secondary suspension damping ($c_s$) & 60 $\times 10^3$\,Ns/m\\
         
         mass per passenger & 70\,kg \\
         train speed & 30 mph (50\,km/h) \\
         track excitation intensity & 1.080 $\time 10^{-6}$\\
         cut-off frequency $\Omega_c$ & 0.8246\,cycles/m\\
         cut-off frequency $\Omega_r$ & 0.0206\,cycles/m \\
         \hline
    \end{tabular}	
\end{table}

The details of a multi-DOF model according to \cite{zhou2009influences} and the derivation of a  corresponding equation of motion is provided in Appendix \ref{appendix:multi_dof}. In matrix form the equation is
\begin{align}
\label{eq:mdof}
\mathbf{M}\ddot{y} + \mathbf{C}\dot{y} + \mathbf{K}y = \mathbf{D_w}z_w + \mathbf{D_{dw}}\dot{z}_w,
\end{align}
where $y$ is a vector of observed parameters, one of which is the vertical displacement $z(x, t)$. $\mathbf{M}$, $\mathbf{C}$ and $\mathbf{K}$ are inertia, damping and spring stiffness matrices respectively, and $\mathbf{D_w}$ and $\mathbf{D_{dw}}$ are the track displacement and velocity matrices. The vertical displacement $z(x, t)$ is a function of space (along the carbody length) and time. 

Vertical track irregularities, $z_w(t)$, is the input to the system described by Eq.~(\ref{eq:mdof}). The output of the system is $z(x, t)$, the vertical displacement of the car as a function of position inside the car. A common approach to modeling the vertical track irregularities is to consider them as a random process with a known power spectral density (PSD). The track PSD depends on the train speed and track quality. For our simulations we use the model described in \cite{hamid1983analytical}:
\begin{equation}
S_{track}(\omega) = \frac{A_v, \Omega_c^2 V^3}{\omega^4 + (\Omega^2 + \Omega^2) V^2 \omega^2 + \Omega_r^2\Omega_c^2 V^4}
\end{equation}
where $\omega = 2 \pi f$ is the circular frequency measured in radians per second, $V$ is the train speed in m/s, $A_v$, $\Omega_c$, and $\Omega_r$ are the track excitation intensity, and the two cut-off frequencies respectively that control the track quality. Parameters $A_v$, $\Omega_c$, and $\Omega_r$ are defined in literature for different track qualities, the values used in our simulation are given in Table \ref{tb:sim-params} and correspond to track grade 2 according to American Railway standard. The corresponding track PSD is shown in Figure \ref{fig:track_psd}.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.65\textwidth]{track_psd.png}
\caption{Power spectral density of track geometry variation.}
\label{fig:track_psd}
\end{figure}

Our analysis looks at the spectral properties of the carbody vertical displacement acceleration at different points along the carbody. Figure~\ref{fig:mdof_psd_center} shows the vertical vibration acceleration PSD  at the center of the carbody. The PSD exhibits prominent peaks around the 1~Hz and 10~Hz regions after which there is a sharp decay. The peak around 1~Hz corresponds to the rigid mode vibration and the peak around 10~Hz corresponds to the flexible mode vibration. Again, each curve in Figure~\ref{fig:mdof_psd_center} represents the acceleration PSD for different passenger loading level indicated in the legend. Comparing the curves shows that the spectral peaks shift towards lower frequency as the passenger loading increases. Also, for a fixed frequency values between 1~Hz and 5~Hz, the magnitude of the PSD decreases for higher passenger loading. Similarly, Figure~\ref{fig:mdof_psd_bogie} shows the vertical vibration acceleration PSD observed above the bogie. The PSD shape is similar to  Figure~\ref{fig:mdof_psd_center}. Again the acceleration PSD changes with increase in the passenger loading.

Clearly there is a correlation between the passenger loading and the spectral properties of the vertical acceleration of the carbody. This change in acceleration PSD should be observable using an accelerometer suitably mounted on board of a carbody. We should be able to infer the current passenger loading from the accelerometer measurements, based on the above results from the multi-DOF train car model.


\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.9\textwidth}
        \includegraphics[width=\textwidth]{mdof_psd_center.png}
        \caption{Above carbody center}
        \label{fig:mdof_psd_center}
    \end{subfigure}
    \hfill
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      
    \begin{subfigure}[b]{0.9\textwidth}
        \includegraphics[width=\textwidth]{mdof_psd_bogie.png}
        \caption{Above bogie}
        \label{fig:mdof_psd_bogie}
    \end{subfigure}
    \caption{Vertical displacement acceleration PSD for the multi-DOF model.}    
    \label{fig:mdof_psd}
\end{figure}

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =

\section{Data driven approach}
The accelerometer based APC will use measurements from the accelerometer sensors suitably placed inside the train car-body. As a part of the Phase I tasks, we planned to collect accelerometer data on operational train cars and perform analysis to see how the data relates to the results from model analysis. In order to conduct the data collection, ARCON implemented an accelerometer datalogger using low-cost open source solutions.

\subsection{Raspberry Pi based datalogger}
The datalogger prototype is implemented using the Raspberry Pi 3 single-board computer with an attached Sense HAT module \cite{raspi3, sensehat}. The Sense HAT module is equipped with a 9 degrees-of-freedom (DOF) IMU sensor. The IMU sensor is capable of recording 3-channel acceleration, angular rate and magnetic field. The Raspberry Pi with the Sense HAT module is powered using a rechargeable battery unit. The Rapsberry Pi with the Sense HAT module and the battery module is placed inside an enclosure creating a self-contained portable datalogger unit. Figure~\ref{fig:logger-topview} shows the internal arrangement of the datalogger unit. We have prepared two such datalogger units for the initial data collection on MBTA subway trains. 

\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\textwidth]{logger_topview.jpeg}
\caption{Top view of the internal arrangement of the Raspberry Pi based datalogger prototype.}
\label{fig:logger-topview}
\end{figure}

The datalogger software operates on the Raspberry Pi and records the IMU measurements at a preset sample rate. At each timestamp, the datalogger records 3D accelerations, 3D angular rates, 3D magnetic field values and the fused 3-D orientation. The recorded values are saved to an on-board SD card and retrieved later for post analysis.

\subsection{Data collection}
ARCON collected data on the subway trains operated by the Massachusetts Bay Transportation Authority (MBTA) \cite{mbta}. We completed several data collection sessions on the MBTA Red Line subway line. Two team members carrying the datalogger units rode the Red Line train cars across several stations \cite{mbta}. The team members placed the datalogger units on the train car floor and initiated data logging. The datalogger units were placed approximately at the center of the train car. Upon departing each station, our team members recorded the approximate passenger count. At the end of each session, the collected data was analyzed.

During each new data collection session, adjustments were made to the data collection procedure based on the lessons learned from the previous session. However after four sessions further data collection was halted for the following reasons,
\begin{itemize}
\item Lack of control over the data collection environment: The team members were riding the subway as normal passengers and hence lacked any control over the data collection environment. It was not possible to guarantee that the logger was placed at the same location on each session. 
\item Improper mounting of the sensors: Accelerometer sensor needs to be properly mounted onto the object whose measurement is desired. But during our data collection sessions, the datalogger was simply placed on the floor without any arrangement to hold it fixed at one position. Without proper mounting, we are unable to ascertain the fidelity of the acceleration measurements recorded. 
\end{itemize}

\subsection{Accelerometer Data Example}
The MBTA Red Line subway line runs in the northwest-to-southeast direction across the Greater Boston region. The northern terminus is the Alewife station and the trains moving away from the Alewife station are considered to be in the \emph{Inbound} direction where as the trains moving towards the Alewife station are considered to be in the \emph{Outbound} direction. 

On August 8, 2017 we conducted four data collection sessions in the inbound and outbound direction between the Alewife station, Davis station, Porter station and the Harvard station. This approach produced three data records per session for inbound and outbound direction respectively. Each data record corresponds to train traveling between two adjacent stations. Table~\ref{tbl:pax_count} lists the approximate passenger count observed during the ride through four stations. Table~\ref{tbl:pax_count_outbound} lists the approximate passenger count observed during the ride in the outbound direction. The first row lists the adjacent stations traversed during the train ride and the first column indicates the approximate starting time for each session.

\begin{table}[!ht]
\centering
\caption{Passenger count during inbound trips}
\label{tbl:pax_count}
\begin{tabular}{|l|l|l|l|l}
\cline{1-4}
         			& Alewife-Davis & Davis-Porter & Porter-Harvard &  \\ \cline{1-4}
Session1 (9:00AM) 	& 20       & 60       & 80       &  \\ \cline{1-4}
Session2 (9:30AM)	& 6        & 12       & 20       &  \\ \cline{1-4}
Session3 (10:30AM)	& 19       & 22       & 25       &  \\ \cline{1-4}
Session4 (11:00AM)	& 10       & 20       & 30       &  \\ \cline{1-4}
\end{tabular}
\end{table}

\begin{table}[!ht]
\centering
\caption{Passenger count during outbound trips}
\label{tbl:pax_count_outbound}
\begin{tabular}{|l|l|l|l|l}
\cline{1-4}
         			& Harvard-Porter & Porter-Davis & Davis-Alewife &  \\ \cline{1-4}
Session1 (9:15AM) 	& 5       & 3       & 5       &  \\ \cline{1-4}
Session2 (9:45AM)	& 45        & 25      & 8       &  \\ \cline{1-4}
Session3 (10:50AM)	& 18       & 13       & 8       &  \\ \cline{1-4}
Session4 (11:30AM)	& 20       & 20       & 4       &  \\ \cline{1-4}
\end{tabular}
\end{table}


Figure~\ref{fig:mbta_accelz} shows the time-series plots of the raw vertical acceleration measurements collected during each session in the inbound direction. The four panels in Figure~\ref{fig:mbta_accelz} correspond to the four sessions mentioned in Table~\ref{tbl:pax_count}. Each time-series plot has segments when the measured acceleration is approximately zero and segments when the measured acceleration is visibly much higher. The latter set of segments correspond to the interval when the train is in motion. As mentioned earlier, when the train is in motion, the track irregularities drive the vertical vibration observed on the train car. In the same spirit, Figure~\ref{fig:mbta_accelz_outbound} shows the time-series plots of the raw vertical acceleration measurements collected during each session in the outbound direction.

% Talk about what we observed in the collected data.
% Some figures and discussion
\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{redline_aug8_vertaccel.png}
\caption{Vertical vibration acceleration measured on MBTA Redline subway train car traveling in the inbound direction from the Alewife station to the Harvard station. Each panel corresponds to a separate data collection session along same set of station}
\label{fig:mbta_accelz}
\end{figure}

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{redline_aug8_vertaccel_outbound.png}
\caption{Vertical vibration acceleration measured on MBTA Redline subway train car traveling in the outbound direction from the Harvard station to the Alewife station. }
\label{fig:mbta_accelz_outbound}
\end{figure}

Figure~\ref{fig:mbta_accelz_psd} shows the PSD of the vertical acceleration measured when traveling from the Alewife to the Porter station (top panel) and traveling from the Porter station to the Davis station. In each panel, the four PSD curves correspond to the data records from the four sessions in Table~\ref{tbl:pax_count}. The legend indicates the passenger count associated with each PSD curve. Comparing the PSD curves in  Figure~\ref{fig:mbta_accelz_psd} and the PSD curves of Figure~\ref{fig:mdof_psd_center} shows the similarity between the acceleration PSD derived from the multi-DOF model and the PSD computed from real data. The PSD in Figure~\ref{fig:mbta_accelz_psd} also has spectral peaks at frequencies corresponding to the rigid mode motion and the flexible mode motion. However, the correlation between the passenger count and the PSD curve is not observable as was the case with the multi-DOF model. It should be noted that the current analysis is based on a very limited set of real data collected from the MBTA subway. Lack of sufficient amount of data impedes us from a statistically valid assessment of the relation between passenger loading and the spectral properties of the vertical acceleration observations of train carbody.

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.8\textwidth}
        \includegraphics[width=\textwidth]{Inbound_station1_psd.png}
        \caption{Alewife to Davis station }
        \label{fig:psd_station1}
    \end{subfigure}
    \hfill
     %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)      
    \begin{subfigure}[b]{0.785\textwidth}
        \includegraphics[width=\textwidth]{Inbound_station2_psd.png}
        \caption{Davis to Porter station}
        \label{fig:psd_station2}
    \end{subfigure}    
    \newpage
%     \begin{subfigure}[b]{0.9\textwidth}
%         \includegraphics[width=\textwidth]{Inbound_station3_psd.png}
%         \caption{Porter to Harvard station}
%         \label{fig:psd_station3}
%     \end{subfigure}
    \caption{PSD of vertical acceleration measured on an MBTA Redline subway train. Each curve corresponds to the passenger loading level indicated in the legend.}
	\label{fig:mbta_accelz_psd}
\end{figure}

\subsection{Issues}
Several issues were encountered during the Phase I effort to establish the proof-of-concept for accelerometer based APC. The major issues are discussed below.

In the model based analysis approach, the multi-DOF train car model requires values for the train car parameters and track geometry spectral parameters listed in Table~\ref{tb:sim-params}. For the analysis presented in Section \ref{sec:mdof}, the parameter values were referenced from \cite{zhou2009influences}. However for a higher fidelity model of a real train car, we need matching parameter values to be used with the model. Such parameter values may be obtained only from manufacturers or operators.
A higher fidelity model will eventually allow us to derive a more accurate algorithm to estimate passenger loading from the accelerometer measurements.

In the data driven approach, our efforts were severely limited by the lack of access to the MBTA train infrastructure. The accelerometer data logger should be securely attached to the train carbody to obtain useful acceleration measurements. When securely attached, we can be certain that (i) all  measurements are from same location on the train car and (ii) improper mounting has minimal impact on the measured data quality. Without any access to the MBTA infrastructure, we are able to obtain only limited data measurements. Moreover since the data logger was simply placed on the carbody floor, we cannot be certain that the accelerometer measurements are not affected by spurious vibrations. 



% \subsection{Recommendation and future actions}

==> datacomm.tex <==
% Chapter reviews data communication systems available
\section{Data communication and PIS}
\label{ch:datacomm}
The proposed CICD system concept in Figure~\ref{fig:cicd_system} shows the three modules connected via data links. The APC sends the on-board passenger count data to the Operations Control Center (OCC) which houses the CICD server. The CICD server computes the expected crowding level on each car for the arriving station. The crowding level information is transmitted to the PIS at the arriving station. This data exchange between the CICD system modules can be achieved using the existing data communication networks used by transit systems. 

All modern rail transit systems use data communication network to support data telemetry between the OCC and the trains, the stations, wayside locations etc. Data telemetry is essential to support operational and safety services such as train control and surveillance. Data telemetry from a train is managed by the on-board telematics system. The telematics system collects data from on-board sensors including the APC and transmits data to the OCC. The on-board sensors and equipment are connected to the telematics system via an in-train network and the data transmission takes place via train-to-wayside communication systems. 

\section{In-train network}
The in-train network connects all the equipment on-board the train cars. On each train car, the on-board equipment are connected to a local network. The train car networks are then coupled together to form the in-train network. The IEEE 1473 standard defines the network protocols to be used for in-train networks. Figure~\ref{fig:intrain} depicts an example of a local network of equipment on a train car. The proposed accelerometer based APC can be connected to the existing telematics system via the in-train network.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\textwidth]{InTrainNetwork.png}
\caption{In-train network}
\label{fig:intrain}
\end{figure}

\section{Train-to-wayside communication}
The train-to-wayside communication (TWC) allows data transport between the moving train and the wayside systems. The wayside equipment are placed along the transit system rail network to support TWC. The TWC system generally use radio links operating a 2.5~GHz or 5.9~GHz (i.e. the ISM band). Major suppliers of data communication network for transit systems have unique products with proprietary protocols for TWC \cite{wayside2013ieee}.

A train traveling between the stations off-loads telemetry data to wayside systems placed along the rail tracks. The wayside systems are generally connected back to the OCC via robust backhaul links. The CICD system will use the existing TWC system and backhaul links to gather APC data from the operating trains.

\section{Passenger Information System}
Passenger information system (PIS) is the automated system used to provide information to the passengers of a transit system. The PIS allows the transit system operators to communicate to the passengers using audio or visual medium. The information provided via PIS can be (i) static information such as service maps and fare (ii) real time information such as current schedule, arrival times, service changes etc. The static information is usually provided in a printed form whereas the real time information is presented on dynamic displays (LCD display) or via audio announcements. 
The elements of the PIS are present on train cars as well as train stations and platforms. The crowding level information generated by the CICD system will be communicated to the awaiting passengers on the dynamic displays present at the station platforms. 

Figure~\ref{fig:mbta_pis} is an example of the PIS at an MBTA train station platform. The PIS consists of three types of displays. On the top left is an array of three LCD panels capable of displaying dynamic media content. On the top right is a monochrome LED display, commonly used for arrival information display. At the bottom are two panels used for printed advertisements. The CICD system can use the LCD panels to display crowding level information for the arriving train. The crowding information will be continually updated for each arriving train. The advertisement panels could be used to inform passengers about the CICD system during the initial roll-out of the system.

Additionally, the modern transit agencies also communicate with the passengers via the agency website, smartphone apps and the social media \cite{mbta, mbta_dev}. These modern communication platform also constitute the PIS. The CICD system crowding level information will be disseminated via  website, smartphone apps. The same information can be made available as a part of the transit agencies' public API collection. The Bay Area Rapid Transit (BART) agency currently provides car crowding level information on the agency website and as a public API \cite{bart,bart_api}.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{mbta_PIS.png}
\caption{The passenger information system (PIS) at an MBTA station platform consists of a digital display (top left), an LED display (top right) and a static advertisement display (bottom)}
\label{fig:mbta_pis}
\end{figure}

The following sections discuss how two transit agencies use the PIS to communicate crowding level information to the passengers.
\subsection*{BART}
In 2013, the Bay Area Rapid Transit (BART) launched a service providing information on the estimated crowding level on trains. The crowding level estimated is not real time, but estimated from the historical ridership data. The estimated crowding level is presented to the passenger using trip planning tool on the BART website \cite{bart}. The crowding level is categorized into three levels indicating “heavy crowding expected,” “moderate crowding expected,” or “light crowding expected.” Each category is indicated by an icon containing three, two and one shadow head-figures as seen in Figure~\ref{fig:bart_crowding}. In the figure, the icons indicates `heavy crowding expected' on the train from Fruitvale to Baboa Park station and `light crowding expected' on the train from Boboa Park station to San Francisco Airport station. Currently, the estimated crowding level is also available to third party developers via the Real BART API \cite{bart_api}.
\begin{figure}[!ht]
\fbox{\includegraphics[width=\textwidth]{crowding_bart.png}}
\caption{A screenshot of the estimated crowding level information displayed by the trip planner tool on the BART website. The crowding level is indicated by icons with shadow head-figures indicating three categories of crowding level.}
\label{fig:bart_crowding}
\end{figure}

\subsection*{Thameslink Railway}
The British Thameslink commuter train service started a service to inform passengers which train cars are most crowded. The crowding level estimates are real time and are based on the ``load weigh system" available on their newest train models Siemens Desiro City Class 700. The real-time crowding level is presented on an overhead display unit inside the train car. The crowding level information is intended for the on-board passengers. The open gangway layout of the train allows the on-board passengers to walk between cars and find a car with less crowding. The displayed crowding level is categorized into four levels `Plenty of Seats', `Carriage Half Full', `Standing Room Only' and `Carriage Full' \cite{desiro}.
\begin{figure}[!ht]
\includegraphics[width=\textwidth]{thameslink_pis.jpg}
\caption{Train crowding level information presented on the Thameslink commuter train. The loading level legends are presented on the left panel and the actual loading levels on each train car is presented on the right panel.}
\end{figure}

==> introduction.tex <==
\section{Introduction}
The Crowding Information Collection and Dissemination (CICD) system is a solution for easing the crowding problem in train cars.  One aspect of the train crowding problem arises due to uneven distribution of the number of passengers in each car in a train consist.  This leads to inefficiency in service and negative passenger experience.  The US Department of Transportation (DOT) published a solicitation requesting innovative solutions to address this particular problem. ARCON proposed a CICD system which aims at addressing this issue by providing the expected crowding level information of each car to the passengers awaiting for boarding that train at the following station. The Phase I effort focused on developing a proof-of-concept (PoC) for the proposed system. Figure.~\ref{fig:schedule} lists the planned tasks for the Phase I effort which spanned the six month Period-of-Performance (PoP) from June to November 2017. At the end of the Phase I PoP, ARCON completed the planned tasks and achieved milestones to develop the PoC for the CICD system. This final report provides a comprehensive overview of the outcomes and accomplishments of the Phase I effort. 

\begin{figure}[!ht]
\centering
\includegraphics[width=0.85\textwidth]{tasks_milestones.png}
\caption{Phase I task schedule for the CICD system}
\label{fig:schedule}
\end{figure}

\section{Phase I outcomes}
The Phase I effort mainly focused on developing the PoC for the modules in the proposed CICD system. ARCON pursued both a data driven and a simulation based approach for the PoC. In the course of scheduled PoP, the proposed tasks were completed and milestones were achieved according to the schedule. The outcomes from the tasks are described below:

\begin{description}
\item[Accelerometer based automatic passenger counter (APC):] ARCON used theoretical model base analysis and accelerometer data from real train cars to demonstrate the feasibility of using accelerometer sensor to infer passenger loading on train cars. An accelerometer sensor datalogger was implemented using a Raspberry Pi computer and a sensor module. The prototype was used to collect real data on the train cars. The analysis of the raw data shows correlation between the train car vibration and passenger loading. Also theoretical model based simulations were conducted to validate the results of the real data analysis.

\item[Passenger Flow Prediction (PFP):] This is a predictive algorithm for inferring boarding and alighting passenger flow from historical data and current APC measurements. ARCON has implemented a prototype PFP algorithm to operate in a simulated simplified train network with a single rail track. Monte Carlo experiments were used to validate the accuracy of the prototype PFP algorithm. Simulation results provide the PoC for using the PFP algorithm to improve the crowding level prediction on train cars.

\item[Technology assessment:] ARCON conducted a high-level technology assessment on current practices for data communication systems and passenger information systems (PIS) in use by rail transit systems. We also reviewed two transit agencies which already provide some form of train crowding information to the passengers.

\item [Deliverables:] ARCON submitted two interim reports with bi-monthly status updates. This final report together with the two previous reports satisfy the deliverables for the Phase I PoP.
\end{description}

% -------------------------- Outline ------------------------------------------------ %
\section{Report outline}
This report is organized as follows: Chapter~\ref{ch:background} reviews the problem of uneven crowding in train cars and describes the proposed CICD system. Chapter~\ref{ch:apc} presents the proof-of-concept for the accelerometer based automatic passenger counter. Chapter~\ref{ch:pfp} presents an overview of our approach for predicting boarding and alighting passenger flow on train cars. A simulation based proof-of-concept is presented. Chapter~\ref{ch:datacomm} presents a high-level survey of the current technology for passenger information dissemination.

==> summary.tex <==
\chapter*{Executive Summary}
\addcontentsline{toc}{chapter}{\numberline{}Executive Summary}%
ARCON proposed the Crowding Information Collection and Dissemination (CICD) system in response to the US Department of Transportation SBIR solicitation on improving the uneven crowding of train cars by providing crowding level information to awaiting passengers. The CICD system Phase I tasks were initiated from June 2017. ARCON has successfully completed all the scheduled tasks and achieved milestones for the Phase I period-of-performance (PoP). This report presents a detailed review of the outcomes of the Phase I tasks.

The CICD system is envisioned to provide information to passengers waiting at a station about the expected crowding level in each car of the arriving train after the passengers alighted at that station. Passengers can use the crowding information to position themselves in front of the car with less expected crowding and thus experience an improved service. The CICD system has a modular design with three main modules: (i) Automatic passenger counting (APC) module, (ii) Passenger Flow Prediction (PFP) module, and (iii) Passenger Information System (PIS). In Phase I, ARCON focused on developing proof-of-concept (PoC) for the APC module and the PFP module.

An automatic passenger counter (APC) is the main source of data for the CICD system. ARCON proposed to develop an accelerometer based APC to measure the passenger loading on train cars. An accelerometer sensor can measure static acceleration like gravity or dynamic acceleration due to the motion or vibration. When properly attached to an object, an accelerometer can be used to measure the dynamic acceleration of the object. The goal of the proposed method is to infer the passenger loading level from the accelerometer measurements on-board a train car. ARCON pursued a simulation based approach and a data driven approach to demonstrate the proof-of-concept for the accelerometer based APC. 
% * <siva1125@hotmail.com> 2017-11-29T19:57:41.008Z:
%
% ^.

The simulation based approach used simplified theoretical models for train carbody to analyze the relation between carbody mass and vertical vibration. The data driven approach focused on gathering accelerometer data from the operational train cars. We have implemented an accelerometer datalogger using a Raspberry Pi computer and a sensor module, which was used to collect data from train cars operating in Boston, MA. A series of theoretical and experimental analyses were conducted to establish a correlation between the carbody vertical vibration and the passenger loading. This correlation between the measurement and passenger loading demonstrates the proof-of-concept for using accelerometer data to estimate passenger loading on a train car. 

ARCON proposed to develop an algorithm to predict crowding level by combining the historical passenger flow data, the current passenger loading, and the predicted passenger flow on each train car. This algorithm is a part of the Passenger Flow Prediction (PFP) module. Instead of simply presenting the APC measured passenger level as the current crowding level, the PFP algorithm aims to predict the expected crowding level after the on-board passengers alight at a station. As a part of the Phase I effort, ARCON developed a prototype PFP algorithm. The prototype PFP algorithm combines the historical data and current APC data using Bayesian inference to predict boarding and alighting passenger flow. The inferred passenger flow is used to predict the expected crowding level. The prototype implementation operates in a simulated train network with a single rail line. Monte Carlo experiments were used to validate the accuracy of the prototype PFP algorithm. Simulation results demonstrate the proof-of-concept for the PFP algorithm.

For the final task, we conducted a high-level technology assessment on current practices for the data communication systems. The three modules of the CICD system need to communicate with each other via the data communication infrastructure used by the train networks. In general, trains have an in-train network on-board to connect all the on-board devices and systems. The APC module can hook on to the in-train network. The train-to-wayside link allows the train to communicate data to the operations control center (OCC). 

We also studied how two transit agencies were using the passenger information system (PIS) to communicate crowding level information to the passengers. The Bay Area Rapid Transit (BART) in California and the Thameslink in London were two transit agencies which provide some form of crowding information to the passengers. In the case of BART, the crowding level information was available only on the website and as a public web API for third party developers. The Thameslink provides crowding information on an on-board display board. This information is intended for the onboard passengers who are allowed to move through the open gangway design to find less crowded area in the train. Neither agency provides crowding information to awaiting passengers at the stations.
